Representations of compact simple Lie groups whose orbit space has non-empty boundary

We provide detailed calculations for the classification of representations of compact simple Lie groups with non-empty boundary in the orbit space, first announced in a previous paper [arXiv:2112.00513] by the same authors.

==> A6.tex <==
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup

\newcommand{\Avi}[6]{
\begin{picture}(6352,895)(1025,-4136)
\thinlines
\put(1201,-3961){\circle{336}}
\put(2401,-3961){\circle{336}}
\put(3601,-3961){\circle{336}}
\put(4801,-3961){\circle{336}}
\put(6001,-3961){\circle{336}}
\put(7201,-3961){\circle{336}}
\put(1369,-3961){\line( 1, 0){864}}
\put(2569,-3961){\line( 1, 0){864}}
\put(3769,-3961){\line( 1, 0){864}}
\put(4969,-3961){\line( 1, 0){864}}
\put(6169,-3961){\line( 1, 0){864}}
\put(1141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{rm}#1}}}
\put(2341,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{rm}#2}}}
\put(3541,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{rm}#3}}}
\put(4741,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{rm}#4}}}
\put(5941,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{rm}#5}}}
\put(7141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{rm}#6}}}
\end{picture}
}

==> A6_15.tex <==
\setlength{\unitlength}{592sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(6352,895)(1025,-4136)
\thinlines
\put(1201,-3961){\circle{336}}
\put(2401,-3961){\circle{336}}
\put(3601,-3961){\circle{336}}
\put(4801,-3961){\circle{336}}
\put(6001,-3961){\circle{336}}
\put(7201,-3961){\circle{336}}
\put(1366,-3961){\line( 1, 0){870}}
\put(2596,-3961){\line( 1, 0){870}}
\put(3796,-3961){\line( 1, 0){870}}
\put(4981,-3961){\line( 1, 0){870}}
\put(6196,-3961){\line( 1, 0){870}}
\put(1141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{5}{6.0}{rm}1}}}
\put(2356,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{5}{6.0}{rm}1}}}
\put(3556,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{5}{6.0}{rm}1}}}
\put(4741,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{5}{6.0}{rm}1}}}
\put(5941,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{5}{6.0}{rm}1}}}
\put(7126,-3451){\makebox(0,0)[lb]{\smash{\SetFigFont{5}{6.0}{rm}1}}}
\end{picture}


==> A6_50.tex <==
\setlength{\unitlength}{1973sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup

\newcommand{\Avi}[6]{
\begin{picture}(6352,895)(1025,-4136)
\thinlines
\put(1201,-3961){\circle{336}}
\put(2401,-3961){\circle{336}}
\put(3601,-3961){\circle{336}}
\put(4801,-3961){\circle{336}}
\put(6001,-3961){\circle{336}}
\put(7201,-3961){\circle{336}}
\put(1369,-3961){\line( 1, 0){864}}
\put(2569,-3961){\line( 1, 0){864}}
\put(3769,-3961){\line( 1, 0){864}}
\put(4969,-3961){\line( 1, 0){864}}
\put(6169,-3961){\line( 1, 0){864}}
\put(1141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}#1}}}
\put(2341,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}#2}}}
\put(3541,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}#3}}}
\put(4741,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}#4}}}
\put(5941,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}#5}}}
\put(7141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}#6}}}
\end{picture}
}

==> Ans_15.tex <==
\setlength{\unitlength}{592sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup

\newcommand{\Ansm}[2]{
\begin{picture}(2752,895)(1028,-4148)
\thinlines
\put(1204,-3973){\circle{336}}
\put(3604,-3973){\circle{336}}
\put(2239,-3958){\circle*{30}}
\put(2389,-3958){\circle*{30}}
\put(2524,-3958){\circle*{30}}
\put(1384,-3973){\line( 1, 0){720}}
\put(2719,-3973){\line( 1, 0){735}}
\put(1159,-3448){\makebox(0,0)[lb]{\smash{\SetFigFont{5}{6.0}{rm}\mbox{$#1$}}}}
\put(3544,-3448){\makebox(0,0)[lb]{\smash{\SetFigFont{5}{6.0}{rm}\mbox{$#2$}}}}
\end{picture}
}
